An efficient combined local and global search strategy for optimization of parallel kinematic mechanisms with joint limits and collision constraints

The optimization of parallel kinematic manipulators (PKM) involve several constraints that are difficult to formalize, thus making optimal synthesis problem highly challenging. The presence of passive joint limits as well as the singularities and self-collisions lead to a complicated relation between the input and output parameters. In this article, a novel optimization methodology is proposed by combining a local search, Nelder-Mead algorithm, with global search methodologies such as low discrepancy distribution for faster and more efficient exploration of the optimization space. The effect of the dimension of the optimization problem and the different constraints are discussed to highlight the complexities of closed-loop kinematic chain optimization. The work also presents the approaches used to consider constraints for passive joint boundaries as well as singularities to avoid internal collisions in such mechanisms. The proposed algorithm can also optimize the length of the prismatic actuators and the constraints can be added in modular fashion, allowing to understand the impact of given criteria on the final result. The application of the presented approach is used to optimize two PKMs of different degrees of freedom.

==> chapters/3rpr.tex <==
\subsection{3 dof 3-RPR mechanism}
\label{subsection:3rpr_implement}
The 3-R\underline{P}R mechanism is a very well known parallel mechanism. It has all the degrees of freedom in $SE(2)$ and can be used for variety of applications and are thus researched widely. The optimisation has been presented by using the interval analysis \cite{bernard_multiobjective_2011}, Nondominated sorting genetic algorithm-II \cite{saadatzi_multi-objective_2011} as well as geometric optimizations \cite{jiang_geometric_2007}. The common objective in all the research is to find a maximum singularity free area. The algorithm presented in this work allows to define an area of interest and if no parameters can satisfy the constraints in the same then the algorithm is capable of returning the best performing parameters after allowing violation. An example is presented to highlight the said advantage of the implementation. The algorithm was set to optimise the parameters for GCI and the reward strategy was biased for center points. It implies that a valid point near the center of the desired workspace had more weightage compared to a valid point near the boundaries of the workspace. This is done to have an optimised results with violations (if any) near the boundaries so that the user has a choice to reduce the space of desired workspace accordingly. The dimension of the optimization space was kept four constraining that all the base points will be equidistant from the center of the mechanism. The parameters optimised are shown in the Fig. \ref{fig:3rprpara}
\begin{figure}[htbp]
    \centering
    \includegraphics[width = 0.4 \textwidth]{images/3rpr_para.eps}
    \caption{The schematic and parameterization of 3-R\underline{P}R}
    \label{fig:3rprpara}
\end{figure}
The options chosen and the range of the parameters are presented in table \ref{table:3RPR_opttable}.
\begin{table}[ht]
    \centering
    \begin{tabular}{c|c|c|c}
        Parameters Value \\ \hline
         Optimization dimension & 4 & Range of $\theta_i$ & [0, $2\pi$]\\\hline
         Range of $r_1$ & [1, 10] & Reward strategy & center biased\\\hline Number of starts & 30 & Number of iterations & 10 and 20\\
         \hline Objective choice & Workspace, GCI & Workspace (rotational) & [-0.261, 0.261]\\\hline
         Workspace (translational)  & square of length 0.6 & stroke ratio & 1.5 \\ \hline 
        Collision constraint & NO & &
    \end{tabular}
    \caption{The parameters set for the optimisation of 3-dof 3-R\underline{P}R mechanism}
    \label{table:3RPR_opttable}
\end{table}
The time required for optimizing this mechanism was comparatively very high. This cleary shows that the dimension of the desired workspace (1 for lambda mechanism, 2 for 2-U\underline{P}S and 3 for 3-R\underline{P}R) has a greater effect on the computational compared to the dimension of optimisation space (1 for lambda mechanism, 13 for 2-U\underline{P}S and 4 for 3-R\underline{P}R). The collision between the legs was not considered in this case as the prismatic joints can be assembled on different heights so that they never collide. The chosen workspace was intentionally kept big to demonstrate the results obtained by accepting the invalid points. The optimisation result for the same are shown in table \ref{table:3RPR_result}. The schematic for the optimised 3RPR mechanism as well as the valid and invalid space in the desired workspace is shown in Fig. \ref{fig:3rp_result}
\begin{table}[ht]
    \centering
    \begin{tabular}{p{7cm}|p{6cm}}
        \hspace{1.5cm}Parameters & Value \\ \hline
        Objective function & Global Conditioning Index  \\ \hline
        Time for 1 coarse evaluation & 450 seconds  \\ \hline
        Time for single coarse start & \alert{In process} \\ \hline
        Time for one fine evaluation & \alert{In process} \\ \hline
        Time for single fine start & \alert{In process}\\ \hline
        Best point &\\$[r_1, \theta_1, \theta_2, \theta_3]$ (refer Fig. \ref{fig:3rprpara})& \alert{[2.6, 2.22, 0, 4.6]} \\ \hline
        Best actuator range & \alert{[2.49, 3.73]} 
    \end{tabular}
    \caption{The results for the optimisation of 3-dof 3-R\underline{P}R mechanism}
    \label{table:3RPR_result}
\end{table}
\begin{figure}[htbp]
    \centering
    \includegraphics[width = 0.8\textwidth]{images/3rpr_results.eps}
    \caption{The schematic plot for the mechanism optimised for GCI and the valid and invalid spaces \alert{WILL BE UPDATED}}
    \label{fig:3rp_result}
\end{figure}


==> chapters/kinematics.tex <==
\section{Kinematic analysis}
    %\addcontentsline{toc}{chapter}{Introduction}	 
    % non-numbered chapters do not appear in table of contents by default
    \label{chapter:kinematics}  

==> chapters/results.tex <==
\section{Results}
    %\addcontentsline{toc}{chapter}{Introduction}	 
    % non-numbered chapters do not appear in table of contents by default
    \label{chapter:results}  
